The intrinsic motivation of reinforcement and imitation learning for sequential tasks

This work in the field of developmental cognitive robotics aims to devise a new domain bridging between reinforcement learning and imitation learning, with a model of the intrinsic motivation for learning agents to learn with guidance from tutors multiple tasks, including sequential tasks. The main contribution has been to propose a common formulation of intrinsic motivation based on empirical progress for a learning agent to choose automatically its learning curriculum by actively choosing its learning strategy for simple or sequential tasks: which task to learn, between autonomous exploration or imitation learning, between low-level actions or task decomposition, between several tutors. The originality is to design a learner that benefits not only passively from data provided by tutors, but to actively choose when to request tutoring and what and whom to ask. The learner is thus more robust to the quality of the tutoring and learns faster with fewer demonstrations. We developed the framework of socially guided intrinsic motivation with machine learning algorithms to learn multiple tasks by taking advantage of the generalisability properties of human demonstrations in a passive manner or in an active manner through requests of demonstrations from the best tutor for simple and composing subtasks. The latter relies on a representation of subtask composition proposed for a construction process, which should be refined by representations used for observational processes of analysing human movements and activities of daily living. With the outlook of a language-like communication with the tutor, we investigated the emergence of a symbolic representation of the continuous sensorimotor space and of tasks using intrinsic motivation. We proposed within the reinforcement learning framework, a reward function for interacting with tutors for automatic curriculum learning in multi-task learning.

==> frontmatter/abstract.tex <==
% the abstract


The challenges posed by  robots operating in human environments on a daily basis and in the long-term point out the importance of adaptivity to changes which can be unforeseen at design time. Therefore, the robot must learn continuously in an open-ended, non-stationary and high dimensional space. It can not possibly explore all its environment to learn about everything within a life-time. 
To be useful and acquire skills, the robot must on the contrary be able to know which parts to sample and what kind of skills are interesting to learn.  One way is to decide what to explore by oneself. Another way is to refer to a mentor. We name these two ways of collecting data \textit{sampling modes}. The first sampling mode correspond to algorithms  developed in the literature in order to autonomously drive the robot in interesting parts of the environment or useful kinds of skills. Such algorithms are called \textit{artificial curiosity} or \textit{intrinsic motivation} algorithms.  The second sampling mode  correspond to \textit{social guidance} or \textit{imitation} where the teacher indicates where to explore as well as where not to explore. Starting from the study of the relationships between these two concurrent methods, we ended up building  an algorithmic architecture where relationships between the two modes intertwine into a hierarchical learning structure, called \textbf{Socially Guided Intrinsic Motivation} (SGIM).

We developed an advanced technique to combine learning by social guidance and intrinsic motivation, for life-long learning of multiple skills. This combination has been designed in a more general context of strategic learning, where the learning agent chooses how to learn best between different learning modes. Our approach enabled the learner to decide online about its interaction with its physical and social environment: what and how to learn; what, when, how and whom to imitate. We will present several implementations of SGIM using different representations and algorithms for its different functions.

Indeed, we have built an intrinsically motivated active learner which learns how its actions can produce varied consequences or outcomes. For instance, the robot learns to throw a ball at different distances, by associating a distance (outcome) to a specific movement (action). It actively learns online by sampling data which it chooses by using several sampling modes. On the meta-level, it actively learns which data collection strategy is most efficient for improving its competence and generalising from its experience to a wide variety of outcomes. The interactive learner thus learns multiple tasks in a structured manner, discovering by itself developmental sequences.
By studying SGIM,  we contribute to different fields of machine learning: 
\begin{itemize}[leftmargin=-.0cm,noitemsep,nolistsep]
\item {\bf imitation learning}:  we explore the questions of \textit{what, how, when and who to imitate}. We propose a unified structure to address simultaneously these fundamental questions of imitation learning. The strategic learner chooses online the options that enable most competence progress. In particular, in {\bf interactive learning} :  we analyse and identify advantages of combining autonomous and socially guided exploration, and build an agent which decides by itself when to interact with teachers.
\item{\bf multi-task learning and goal-directed learning}: SGIM can discover the structure of its environment by a goal-oriented exploration. %In classical approaches, goal-directed learning approaches have been studied in autonomous learning  as a way to focus on different goals to guide policy exploration. In contrast, in imitation learning, efforts have focused more on goal understanding or  intentionality. Here 
We propose a unified architecture to approach goal-oriented imitation learning and goal-directed autonomous exploration.
\item {\bf active learning}: we investigate different levels of active learning: the learner decides  which action to take, which goal to aim, and which mode to perform. Its decisions are made online, driven by artificial curiosity based on its monitoring of the learning progress.
\item {\bf hierarchical learning}: we propose a hierarchical learning architecture to learn on several levels: policy, outcome, and sampling mode.  The learner relies on hierarchical active decisions of what and how to learn driven by empirical evaluation of learning progress.% for each sampling mode on a meta-level. 
\end{itemize}

\footnotesize{
This thesis is structured as follows. We first formalise in Chapter 1 a computational framework in the context of cognitive developmental robotics. This is a field which both builds efficient robot learners using inspiration from cognitive science and developmental psychology, and  models and tests cognitive science and developmental psychology theories using robotic learners.  In Chapter 2, we illustrate the question we address in our computational framework with an experiment where the iCub robot learns to recognise 3D objects by manipulation. Then we present successively three algorithmic architectures, each one allowing the agent to take more active control of its learning strategy. We have built  these  algorithms for quick and accurate multi-task learning, grounding their designs on developmental studies of intrinsic motivation and imitation learning.
Firstly, we  design an algorithmic architecture which learns \textit{what and how to learn}, called  Socially Guided Intrinsic Motivation by Demonstration (SGIM-D). It actively explores policy and outcome spaces using both imitation learning and goal-oriented autonomous exploration. The design of SGIM-D allows an analysis of the complementarity between these two sampling modes.
Secondly, we explore the question of  \textit{when to imitate} by  additionally actively learning which of the two sampling modes to use.  Our new system, called SGIM with Interactive learning at the Meta level (SGIM-IM) allows the interactive learner to actively and hierarchically explore the policy, outcome, and also sampling mode space.
Finally, we extend SGIM-IM into a system which learns \textit{how, when, what and who to imitate}.  SGIM with Active Choice of Teacher and Strategy (SGIM-ACTS) is a complete active learner, deciding on all aspects of its strategic learning. It extends SGIM-D and SGIM-IM. SGIM-ACTS considers the case when more teachers are available and more modes can be chosen.
%The first one presented in Chapter 3, called for Socially Guided Intrinsic Motivation by Demonstration (SGIM-D), actively explores policy and outcome spaces using both imitation learning and autonomous exploration. The design of SGIM-D allows an analysis of the complementarity between these two sampling modes. SGIM-D thus answers the questions of \textit{what and how to learn}.
%The second one, called SGIM with Interactive learning at the Meta level (SGIM-IM), allows the interactive learner to actively explore the policy, outcome, and also sampling mode space. SGIM-IM learns  \textit{when to imitate} by  additionally choosing actively which of the two sampling modes to use.  The third one, called SGIM with Active Choice of Teacher and Strategy (SGIM-ACTS), extends SGIM-IM and considers this active choice when more teachers are available and more modes can be chosen. SGIM-ACTS explores the questions of \textit{how, when, what and who to imitate}.  
SGIM-IM and SGIM-ACTS  are described in Chapter 4.
Finally, while in the previous chapters we aimed at building artificial systems for autonomous life-long learning, chapter 5 shows that the developed architecture can be useful to model and understand better infant development. We use the developed algorithms to study an observation in child psychology: the development of vocalisation in babies. We illustrate how  an embodied agent using SGIM-ACTS can learn to vocalise and the emergence of a developmental sequence. This work also shows that the algorithmic architecture SGIM-ACTS can be instantiated with another representation of a model and  another optimisation algorithm. In conclusion, the limits and possible extensions of these contributions are discussed in Chapter 6.}

\vspace{0.5cm}
\footnotesize{
\textbf{Keywords : 
active learning,
interactive learning, 
imitation learning, 
goal-oriented exploration, 
data-collection, 
exploration, 
programming by demonstration
}
}



%%%%%%%%%%%%%%%%            COMMENT  %%%%%%%%%%%%%
\begin{comment}

\textbf{Contributions}

\begin{itemize}
\item {\bf With SGIM we have obtained} : an intrinsically motivated active learner who learns to achieve various outcomes by generalising from data samples which it chooses by using several learning strategies: autonomous exploration or socially guided exploration. The interactive learner chooses at a meta-level actively and adaptively which learning strategy enhances learning best.


\item {\bf SGIM made contributions in these fields} : 
\begin{itemize}
\item {\bf imitation learning} : We explore the questions of what, when and who to imitate.
\item {\bf interactive learning} : We analyse and identify advantages of combining autonomous exploration and socially guided exploration.
\item {\bf goal-directed learning} : until now, goal-directed learning approaches have been studied in autonomous learning and imitation learning very differently. In the former case, it is about focusing on a goal to guide policy exploration. In the latte case, efforts have focuses more on goal understanding or  intentionality. Here we propose a unified architecture to approach imitation learning and goal-directed autonomous exploration.
\item {\bf active learning} :  To choose which strategy with a new measure nased on intrinsic motivation (comeptence progress). 2nd point: we choose both the task and the strategy at the same time.
\item {\bf hierarchical learning} : we propose a hierarchical learning architecture to learn on several levels: policy, outcome, and strategy spaces.
\item{\bf multi-task learning} : learn how to generalise from already know tasks to achieve new tasks.
\end{itemize}
\end{itemize}



Learn motor skills to achieve various outcomes with different data-collection strategies
Can generalise for new outcomes
in complex, high-dimensional, continuous spaces
goal-directed learning, exploration
Mixing social guidance and self-guided exploration
interactive learner: what, when, who

goal-directed interactive learning/ interactive goal-babbling/interactive goal-directed learning


\textbf{Outline}

The strategic learner consists in an agent who learns a mapping M:A->B by deciding at each timestep which sub-mapping Mb:A->{b} to learn (goal-directed learning) and which data collection strategy to use [explain this directly with the illustration of obj recognition]. Example of strategies that are popular are intrinsic motivation and social guidance. Illustration on the iCub object recognition of 3d objects.

The pb of active data collection is all the more acute in complex continuous environments: explain M:A->B for continuous spaces, pb redundancy, unboundedness, lifelong learning.
Most popular solutions are intrinsic motivation and social guidance, but they have their limits.  Combining them can improve performances. Ex of SGIM-D with ICDL2012 paper.

Once we have proved their combination is beneficial, we make active versions of it: SGIM-IM and SGIM-ACTS.

Then we illustrate this on a developmental ex.

\newpage

\textbf{Outline1}

The strategic learner consists in an agent who learns a mapping M:A->B by deciding at each timestep which sub-mapping $M_{sub}$ he should learn and which data collection strategy to use. 

1.1.To explain the problem, we illustrate with a simple problem where you learn to recognise 3d objects with all its different views.
1.1.1. We introduce the questions of: which strategy to use, which object to learn about.
1.1.2. This is an interesting question because few works have addressed both questions at the same time.

1.2. Active learning
explain what is active learning compared to passive learning, selection of data, principle of limited time vs cost in time for each sampling

1.3. We also introduce the notion of goal-oriented learning, and teleological learning.
we could just decide what image to choose, or, instead choose which  which object to manipulate, i.e. about which object to learn more. This is about goal-oriented learning.
More generally : Teleological learning, [context][action][outcome]

1.4. We formalise this problem while considering continuous spaces. (illustrate directly with the icub experiment or also use the tennis example?)

1.5. Experiment with the iCub: we illustrate how to solve this problem in the case of discrete spaces, and show results.

2. What if we learn more complicated mapping? We consider mapping where A and B are continuous and we wish to learn inverse models with high redundancy. 

2.1 Pbs of life-long learning: redundancy, stochasticity, continuous spaces, high-dimensional spaces, limited nb of experiments/data.

2.2. Social Guidance 
is a classical approach to life-long learning. 

2.2.1. The principle of social guidance and a few successful studies.

2.2.2. Analysis of Social Interaction Modes : 
There are a lot of approaches, which can be analysed by  the who what when how questions.

2.3. Intrinsic Motivation
is a new approach to life-long learning.

2.4.1. Combining Social Guidance and Intrinsic Motivation
should be a good idea because they enable to overcome the other's limits

2.4.2. SGIM-D
This is why we designed SGIM-D, which we describe in detail.

2.4.3. Application to a case study: the fishing rod experiment
we describe the experimental setup
and the algorithm for this case study.

2.4.4. Experimental Protocol

2.4.5. Experimental Results

2.4.6. Analysing the influence of demonstrations
Demonstrations bias the exploration of policy space and outcome space.

2.4.6. Conclusion for SGIM-D
SGIM-D is successful, so it makes sense to consider social guidance and intrinsic motivation as complementary strategies.  
But still it is a passive system with only 1 type of outcomes and 1 teacher. We make now an active version of it.

3. Interactive Strategic Learner

3.1. what is interactive learning, and their benefits

3.2. SGIM-IM
we build a simple strategic learner in the case of only 2 strategies. It can adjust by itself to the right amount of necessary demonstrations. we address the question when to imitate

3.2. 
what if we have more strategies, and more teachers. We address what and who to imitate

3.3. Illustration on a developmental sequence for vocalisation

4. Conclusion
We identified the pb of strategic learning, which is more crucial for complex, continuous, redundant, stochastic environments.
We identified two families of learning algorithms, and used them as strategies.
We first illustrated that it can learn efficiently in the case of a simple mapping to learn, then a more complex one, and finally that developmental trajectories can emerge.

4.1. Contributions

Learn motor skills to achieve various outcomes with different data-collection strategies
Can generalise for new outcomes
in complex, high-dimensional, continuous spaces
goal-directed learning, exploration
Mixing social guidance and self-guided exploration
interactive learner: what, when, who

goal-directed interactive learning/ interactive goal-babbling/interactive goal-directed learning

We built a strategic learner architecture to learn 
- in both robotic setups and simulations
- mappings with discrete spaces and continuous redundant spaces
- with learning paradigms of intrinsic motivation and social guidance

4.2. Extensions
context
build complex actions like Barto




\newpage

\textbf{Outline2}

1.1.1. Life-long learning for open-ended cognition in changing environments is a difficult problem: redundancy, stochasticity, continuous spaces, high-dimensional spaces, limited nb of experiments/data. And most classical optimisation approaches learn for one particular task, predesigned by the engineer.

1.1.2. Developmental cognitive approaches, taking inspiration from developmental psychology and neurosciences, propose good methods. Principles of learning, embodiment, development, trial and error ... are bases of our work.

1.1.3. Active learning: explain what active learning is, compared to passive learning(selection of data, principle of limited time vs cost in time for each sampling). sensori-motor loop, enactment, trial and error : action is essential to learning/prediction of sensors. 

1.2. Several methods have thus been built, but each of them have limitations :

1.2.1. Intrinsic motivation: artificial curiosity, inspired by psychology theories of flow, have given many efficient methods.
IAC, SAGG-RIAC

1.2.2. Teleological learning: goal-babbling, which gets inspired from experiments showing that children have expectancies about outcomes. [context][action][outcome].

1.2.3. Social guidance : direct transfer from human to robot. Several types of social guidance : analysis of social interaction modes by the who what when how questions (illustrate with the tennis pb).

1.3.  Limitations of each of the methods taken separately

1.3.1. Limitations of social guidance

1.3.2. Limitations of intrinsic motivation

1.3.3. Combining them can enable to overcome each other's limits.
 
1.4. Strategic learning
we can consider these mechanisms as strategies and study them together instead of studying them separately. We study how intrinsic motivation, social guidance, and goal-babbling can be combined into an efficient algorithm.

1.4.1. What to learn and how to learn
this problem has been formalised under the notion of strategic learning. Few approaches have considered the question of what to learn and how to learn, these questions have been studied separately so far.

1.4.2. Formalisation
we formalise the pb in the general case (and illustrate with the tennis example).

2. Strategic learning of a classification pb : the iCub experiment.
We illustrate with a simple classification pb where the icub robot learns to recognise 3d objects by manipulation.

3. What if we learn more complicated associations in continuous, high-dimensional spaces.

3.1. SGIM-D: this is why we designed the passive SGIM-D algorithm and describe it.

3.2. Application to a case study: the fishing rod experiment: we describe the experimental setup and the algorithm for this case study.

3.3. Experimental Protocol

3.4. Experimental Results

3.5. Analysing the influence of demonstrations: demonstrations bias the exploration of policy space and outcome space.

3.6. Conclusion for SGIM-D: SGIM-D is successful, so it makes sense to consider social guidance and intrinsic motivation as complementary strategies. But still it is a passive system with only 1 type of outcomes and 1 teacher. We make now an active version of it.

4. Interactive Strategic Learner

4.1. what is interactive learning, and their benefits

4.2. SGIM-IM :
we build a simple strategic learner in the case of only 2 strategies. It can adjust by itself to the right amount of necessary demonstrations. we address the question when to imitate

4.3. SGIM-STRATS :  
what if we have more strategies, and more teachers. We address what and who to imitate

We have built efficient algorithms for learning.

5. Illustration on a developmental sequence for vocalisation
Until now, we have developed an efficient algorithm. But we illustrate that it can reproduce a developmental trajectory, and model child development.

6. Conclusion
We identified the pb of strategic learning, which is more crucial for complex, continuous, redundant, stochastic environments.
We identified two families of learning algorithms, and used them as strategies.
We first illustrated that it can learn efficiently in the case of a simple mapping to learn, then a more complex one, and finally that developmental trajectories can emerge.

6.1. Contributions

Learn motor skills to achieve various outcomes with different data-collection strategies; 
Can generalise for new outcomes;
in complex, high-dimensional, continuous spaces;
goal-directed learning, exploration;
Mixing social guidance and self-guided exploration;
interactive learner: what, when, who

goal-directed interactive learning/ interactive goal-babbling/interactive goal-directed learning

We built a strategic learner architecture to learn  : 
- in both robotic setups and simulations
- mappings with discrete spaces and continuous redundant spaces
- with learning paradigms of intrinsic motivation and social guidance

6.2. Extensions: 
context, 
build complex actions like Barto



\end{comment}










==> frontmatter/abstractfr.tex <==
% the abstract

blablah





\footnotesize{
\vspace{0.5cm}
\textbf{Mots clés : 
collecte de données, 
apprentissage actif,
imitation active,
s\'equence de mouvements,
apprentissage continu,
apprentissage hi\'erarchique,
apprentissage int\'eractif,
apprentissage par imitation,
exploration orientée par objectifs, 
exploration, 
apprentissage par d\'emonstration
}
}










==> frontmatter/authorlist.tex <==
\noindent The following authors contributed to Chapter 1: Sao Mai Nguyen.

\noindent The following authors contributed to Chapter 2: Sao Mai Nguyen.

\noindent The following authors contributed to Chapter 3: Sao Mai Nguyen. 


==> frontmatter/committee.tex <==
\footnotesize
%{\bf Jury:} \\
%\vspace{1em}\\	
\onehalfspacing
\begin{tabular}{l l l l }
 
{\bf Thesis Rapporteurs} \\
 Prof.~{\sc  Lola Cañamero}  & ETIS Lab CY Cergy Paris Université%, ENSEA, CNRS UMR8051 
 & Director \\
%Thesis Rapporteur 
 Prof.~{\sc  Mohamed Chetouani}  & Institut des Systèmes Intelligents et de Robotique%, 
%CNRS UMR7222 
& Adjunct Director \\
%Thesis Rapporteur \\
 Dr.~{\sc Sylvain Calinon}  & Idiap Research Institute, 
Switzerland & Senior Research Scientist \\
\\
{\bf Jury President : }\\
 Prof. ~{\sc   Richard Duro}  & Universidade da Coruna & Professor\\
\\
{\bf Jury Member : }\\
 Pr.~{\sc  Jun Tani}  & Okinawa Institute of Science
and Technology & Professor\\
 
\end{tabular}


==> frontmatter/dedication.tex <==
% dedication text
\begin{flushright}
Xin chân thành cảm ơn bố mẹ \\
Nguyễn Bá Hào \\
và \\
Đặng Thị Thu Oanh
\end{flushright}

==> frontmatter/resume.tex <==
My work in the field of developmental cognitive robotics aims to devise a new domain  bridging between reinforcement learning and imitation learning, with \textbf{a model of the intrinsic motivation for learning agents to learn  with guidance from tutors multiple tasks, including sequential tasks}.  My main contribution has been to propose a	 common formulation of intrinsic motivation based on empirical progress for a learning agent to choose automatically its learning curriculum by actively choosing its learning strategy for simple or sequential tasks:  which task to learn, between autonomous exploration or imitation learning, between low-level actions or task decomposition, between several tutors. The originality is to design a learner that benefits not only passively from data provided by tutors, but to actively choose when to request tutoring and what and whom to ask. The learner is thus more robust to the quality of the tutoring and learns faster with fewer demonstrations.

With my previous advisors, colleagues and my collaborators, we developed the framework of \textbf{socially guided intrinsic motivation} with machine learning algorithms to learn multiple tasks by taking advantage of the generalisability  properties of human demonstrations  in a passive manner   
or in an active manner through requests of demonstrations from the best tutor for simple   
and composing subtasks.
The latter relies on a representation of subtask composition  proposed for a construction process, which should be refined by representations used for observational processes of analysing human movements and activities of daily living.  With the outlook of a language-like communication with the tutor, we investigated the emergence of a symbolic representation of the continuous sensorimotor space  and of tasks    using intrinsic motivation. 
These works proposed within the reinforcement learning framework, a \textbf{reward function for interacting with tutors} for multi-task learning. The formulation of this reward unifies interactive learning, multi-task learning and hierarchical learning through the same empirical competence progress measure as the intrinsic motivation to choose the different aspects its  learning strategy.

The socially guided intrinsic motivation framework could be used for intelligent tutoring systems  to be applied in socially assistive robotics 
for a robot coach for physical rehabilitation of low-back pain patients analysing whole body movements, or for a robot coach for ASD children in an imitation game.   

The project I wish to develop in cognitive developmental learning pertains both to the reinforcement learning framework of machine learning, to control learning in the perception-action loop of cognitive robotics and  the theory of intrinsic motivation from developmental psychology in cognitive science. The objective is to propose new reinforcement learning algorithms for robots to learn by actively interacting with their environment, enabling robots to master control tasks of growing complexity, while extending the current theory of intrinsic motivation towards a unified model of motivations for interacting with tutors. The project relies on two axes : a model of interaction with tutors relying on an emerging representation of tasks by the robot, and a model of motivation of human learners through the use case of a robot coach for physical rehabilitation. This work will enrich the formulation of the motivation for social guidance with various motivational drives of learners to interact with tutors, taking the perspective of communication and emotions. This will also highlight the importance of emerging internal representations for understanding social guidance, thus emphasising the interdependence between autonomous learning and social learning.

\vspace{1em}

\textbf{Keywords} : Interactive Reinforcement Learning, Active Imitation Learning, Social Guidance, Intrinsic Motivation, Reinforcement Learning, Hierarchical Learning, Human Movement Analysis, Activities of Daily Living, Activity Recognition, Socially Assistive Robotics, Smart Home

==> frontmatter/resumefr.tex <==
Ma recherche dans le domaine de la robotique cognitive développementale cherche à concevoir un nouveau domaine qui allie apprentissage par renforcement et apprentissage par imitation, avec un modèle de motivation intrinsèque pour que des agents apprennent plusieurs tâches, dont des tâches séquentielles, avec la guidage de tuteurs. Ma principale contribution a été de proposer une formulation commune de la motivation intrinsèque, basée sur le progrès empirique, pour qu'un agent choisisse automatiquement son programme d'apprentissage en choisissant activement sa stratégie d'apprentissage pour des taches simples ou séquentielles :  la tâche à apprendre;  le tuteur à imiter; stratégie entre exploration autonome ou apprentissage par imitation, entre des actions bas niveau ou une décomposition de taches. 
L'originalité est de concevoir un agent d'apprentissage qui bénéficie non seulement passivement des données provisionnées par des tuteurs, mais aussi en choisissant activement quand demander de l'aide et quand et à qui demander. L'apprenant est ainsi plus robuste à la qualité du tutorat et apprend plus vite avec moins de démonstrations.

Avec mes encadrants, collègues et collaborateurs, nous avons développé le cadre de la \textbf{motivation intrinsèque guidée socialement}  des algorithmes d'apprentissage multi-tâches, en profitant des propriétés de généralisation des démonstrations par des humains observées de manière passive ou de manière active par le biais de requêtes au meilleur tuteur de démonstrations pour des taches simples ou pour composer des tâches complexes. Cet apprenant exploite des représentations de composition de sous-tâches que nous proposons pour une démarche constructiviste, et qui devrait être précisées par des représentations utilisées pour des démarches observationnelles comme l'analyse de mouvements humains et d'activités de la vie quotidienne. Dans la perspective d'une communication par un pseudo-language avec le tuteur, nous avons étudié l'émergence de représentations symboliques de l'espace continu sensorimoteur et des taches, grâce à la motivation intrinsèque. Nos travaux ont proposé dans le cadre de l'apprentissage par renforcement, une \textbf{fonction de récompense pour interagir avec des tuteurs} pour l'apprentissage multi-taches. La formulation de cette récompense unifiant l'apprentissage interactif, l'apprentissage multi-taches et l'apprentissage hiérarchique, au travers de la même mesure empirique de progrès en compétence, comme motivation intrinsèque pour choisir les différents aspects de sa stratégie d'apprentissage.

Ce cadre de la motivation intrinsèque guidée socialement pourrait être utilisée pour les systèmes de tutorat intelligent, pour être appliquée en robotique d'assistance sociale, pour un robot coach pour la rééducation physique pour des patients de lombalgie qui analyse les mouvements corporels, ou pour un robot coach pour des enfants ayant un TSA dans des jeux d'imitation. 

Le projet que j'aimerais développer en apprentissage cognitif développemental se rapporte à la fois au cadre de l'apprentissage par renforcement en apprentissage automatique, pour l'apprentissage du contrôle dans une boucle action-perception de la robotique cognitive, et de la théorie de la motivation intrinsèque  qui provient de la psychologie développementale in science cognitive. L'objectif est de proposer de nouveaux algorithmes d'apprentissage par renforcement pour permettre aux robots d'apprendre en interagissant de manière active dans leur environnement, en permettant aux robots de maitriser des tâches de contrôle de complexité croissante, tout en développant la théorie actuelle de la motivation intrinsèque pour un modèle unifié des motivations à interagir avec des tuteurs. Le projet s'appuie sur deux axes de recherche : un modèle d'interaction avec des tuteurs reposant sur une représentation émergente des tâches; et un modèle de la motivation des apprenants humains à travers le cas d'un robot coach pour la rééducation physique. Ce travail va enrichir la formulation de la motivation pour le guidage social avec différentes impulsions motivationnelles des apprenants pour interagir avec des tuteurs, en adoptant le point de vue de la communication et des émotions. Ceci va aussi mettre en lumière l'importance de représentations internes émergentes pour la compréhension du guidage social, ainsi souligner l'interdépendance entre apprentissage automatique et apprentissage social.


\vspace{1em}


\textbf{Mots clés} : Apprentissage par renforcement interactif, Apprentissage par imitation actif, Guidage social, Motivation Intrins\'eque, Apprentissage par renforcement, Apprentissage hi\'erarchique, Analyse de movement humain, Activit\'es de la vie quotidienne, Reconnaissance d'activité

==> frontmatter/thanks.tex <==
% the acknowledgments section
 
 

==> pseudocode/PseudoCodeExecuteSGIMD.tex <==

\begin{algorithm}
\caption{ [$(a,b,c)$] = Execute($c, b$) \\ Set context $c$ and perform policy parameters $b $ }
\zlabel{alg:Execute}
\begin{algorithmic}[1]
\STATE{ Initialise robot at $c $  }
\STATE{Perform policy of parameters $b$.}
\STATE{Measure outcome $a$ in the outcome space} 
\STATE{$flagInteraction  \gets $ check for a teacher's demonstration}
\RETURN  $(a,b,c)$
\end{algorithmic}
\end{algorithm}


==> pseudocode/PseudoCodeExplorationSGIMD.tex <==
 \begin{algorithm}
 \caption{[$\mathcal{D}$] = Goal-Directed Policy Optimization($c,a_g, p(b|a), \mathcal{H}$). \\ Search for policies to reach $a_g$ in context $c$ while building model}
 \zlabel{alg:PseudoCodeExploration}
\begin{algorithmic}[1]
\STATE{{\bfseries Initialise:} $\mathcal{D} \gets $ empty list of $(c, b,a)$}

   \STATE{$(a_{close}, b_{close}, c_{close} ) \gets $ Search in $\mathcal{H}$ for the  $a_{close}$ closest to $a_g$}
	        \STATE{ $mLow \gets$  mode \textit{global-exploration} or \textit{local-optimization} with probability   $\propto J(a_g, b_{close}, c_{close})$}
  \IF{ $mLow$ =  \textit{global-exploration} }
	        \STATE{Action parameter $a \gets$  random movement parameters}   \zlabel{line:randomMovement}
	       % \STATE{ Initialise robot at $(x_{org},y_{org}) $ }
	        \STATE{$(c,b,a) \gets $  \textsf{ Execute}($c, b$)}  \zlabel{line:executeGDPO}
	        \STATE{Add $(a,b,c)$ to $\mathcal{D}$ }
	       % \STATE{Measure new state $(x_2,y_2)$  and memorise $(x_{org},y_{org}, a,x_2,y_2)$ }
	  \ELSIF{ $mLow$ =   \textit{local-optimization}}
	     \STATE{$\mathcal{D} \gets $ \textsf{LocalOptimization}($c,a_g, p(b|a), \mathcal{H}$) }                                \zlabel{line:localOptimisation}
	  \ENDIF
\RETURN{$\mathcal{D}$}
\end{algorithmic}
\end{algorithm}

==> pseudocode/PseudoCodeImitationSGIMD.tex <==
 \begin{algorithm}
 \caption{ [$\mathcal{D}$] = Mimic Policy($b_{d},c$)}
 \zlabel{alg:PseudoCodeImitation}
\begin{algorithmic}[1]
\STATE {{\bfseries Input:} $nIm$ : duration of the imitation phase;}
\STATE {{\bfseries Input:} thresholds:  $\epsilon_{max}$; }
\STATE{{\bfseries Initialise:} $\mathcal{D} \gets $ empty list of $(a,b,c)$}
  	\FOR{$nbMimic$ times}
	\STATE{$b_{rand} \gets$  random vector such that $|b_{rand}|< \epsilon_{max}$}   \zlabel{line:randImitate} 
	\STATE{$b \gets b_{d} + b_{rand}$  }
	\STATE{$(a,b,c) \gets $ \textsf{ Execute} ($c,b$)}
	\STATE{Add $(a,b,c)$ to $\mathcal{D} $}
	\ENDFOR
\RETURN{$\mathcal{D}$}
\end{algorithmic}
\end{algorithm}

==> pseudocode/PseudoCodeLocalDataSGIMD.tex <==
\begin{algorithm}
\caption{ [$K_{l_{best}} $] = LocalData($ a_g,\mathcal{H}$). \\ Retrieve from the memory $\mathcal{H}$ experiences in the locality of $a_g$  }
 \zlabel{alg:LocalData}
\begin{algorithmic}[1]
\STATE{ {\bfseries input}: thresholds distM, distN }
\STATE{Get from the memory the nearest neighbours of $a_g$: }
\STATE{$ H \gets \{(a_h, b_h, c_h) \in \mathcal{H} |  \left\{
\begin{array}{rl}
J(a_g,b_h,c_h) <distM & \\
J(a_g,b_h,c_h) < J(a_h,b,c) , \forall (a,b,c) \in \mathcal{H} - H\\ 
 \end{array} \right.
 \} 
 $                  \zlabel{line:localDataH} }
\STATE{$\forall (a_h,b_h,c_h) \in L$, $K_l \gets \{(a,b,c)\in \mathcal{H}| ||b-b_h|< distN \} $ }                                    \zlabel{line:localDataK}
\STATE{Select the best locality :$ l_{best} \gets argmin(\textsf{LocalQuality}(K_l,a_g) $)}  \zlabel{line:localDataR}
\RETURN{ $K_{l_{best}} $}
\end{algorithmic}
\end{algorithm}


==> pseudocode/PseudoCodeSGIMACTS.tex <==
\begin{algorithm}
\caption{SGIM-ACTS}
\zlabel{alg:PseudoCodeSGIMACTS}
\begin{algorithmic}
\STATE  {\bfseries Input:}  the different modes $ \chi_\alpha,...  \chi_{\kappa}$. %($\chi_1$ is intrinsic motivation).
\STATE  {\bfseries Initialization:} partition of outcome space $\mathcal{R } \gets $  singleton $ A$
\STATE  {\bfseries Initialization:} episodic memory (collection of produced outcomes) $\mathcal{H} \gets$  empty memory
\STATE  {\bfseries Initialization:} $e \gets 1$

\LOOP

\STATE{ $a_i,\chi \gets \textsf{Select Goal Outcome and Sampling Mode}(\mathcal{R } )$}
  \IF{\underline{$\chi = $ Mimic teacher $i$ mode}}              \zlabel{line:ACTSMimic}
  \STATE{ $ (\zeta_d,a_d) \gets$ ask and observe demonstration to teacher $i$. }
 % \STATE{\textsf{Emulation}: $a_g \gets a_{d}$ }%and the context $c \gets c_{demo}$ }
             \STATE{$\gamma_1 \gets$ Competence for $a_g$  }	
        \STATE{ $\mathcal{D}_e  \gets {\textsf{Mimic Action}} (\zeta_{d}$) }
    \STATE $p_{e+1} \gets \mathcal{L}(p_e,\mathcal{D}_e)$ 
            \STATE{$\gamma_2 \gets$ Competence for $a_g$  }

  \ELSIF{\underline{$\chi =$ Emulate teacher $i$ mode}}  \zlabel{line:ACTSEmulation}
  \STATE{ $ (\zeta_d,a_d) \gets$ ask and observe demonstration to teacher $i$. }
  \STATE{\textsf{Emulation}: $a_g \gets a_{d}$ }%and the context $c \gets c_{demo}$ }
             \STATE{$\gamma_1 \gets$ Competence for $a_g$  }	
    \STATE{ $\mathcal{D}_e   \gets {\textsf{Goal-Directed Policy Optimisation}}(a_g) $}
    \STATE $p_{e+1} \gets \mathcal{L}(p_e,\mathcal{D}_e)$ 
            \STATE{$\gamma_2 \gets$ Competence for $a_g$  }

  \ELSE
  \STATE{ \textbf{\underline{$\chi = $ Intrinsic Motivation mode}}} \zlabel{line:ACTSAuton}
   \STATE{\ $a_g \gets a_{i}$ }%and the context $c \gets c_{demo}$ }
               \STATE{$\gamma_1 \gets$ Competence for $a_g$  }	
  \STATE{$ \mathcal{D}_e  \gets {\textsf{Goal-Directed Policy Optimisation}}(a_g) $}
    \STATE $p_{e+1} \gets \mathcal{L}(p_e,\mathcal{D}_e)$ 
        \STATE{$\gamma_2 \gets$ Competence for $a_g$  }
\ENDIF

\STATE{$nbA \gets \textsf{number of  episodes in } \mathcal{D}_e$}
\STATE{$prog \gets  2( sig(\alpha_p* \frac{\gamma_2 -\gamma_1}{|T_i| \cdot nbA}) -1 )$  }
 \STATE{ Append $\mathcal{D}_e $ to $\mathcal{H}$ }
 \STATE{ $\mathcal{R } \gets \textsf{ Update Outcome and Sampling Mode Interest Mapping}(\mathcal{R },\mathcal{H},a_g,prog, \chi)$}
\STATE{$e \gets e+1$}
\ENDLOOP	  
\end{algorithmic}
\end{algorithm}

==> pseudocode/PseudoCodeSGIMACTSIcub.tex <==
\begin{algorithm}

\caption{SGIM-ACTS for Discrete Outcomes Spaces}

\zlabel{alg:PseudoCodeSGIMACTSIcub}

\begin{algorithmic}[1]
\STATE  {\bfseries Input:} $s_1, s_2, ...$ : available sampling modes with cost $\kappa_i$.
\STATE  {\bfseries Initialization:} $\mathcal{R } \gets $  singleton $\{B\}$.
\STATE  {\bfseries Initialization:} $\mathcal{H} \gets$  empty episodic memory of sets of associations (a,b).

\LOOP
%\STATE{ $\chi_i,b_g \gets \textsf{Select Label and Mode}(\mathcal{R } )$}
\STATE{ $\chi_i,b_g \gets \textbf{Select Label and Sampling Mode}(\mathcal{R } )$}
\REPEAT
\IF{ $\chi_i$ is a Social Guidance learning mode}
  \STATE{ $(a_r,b_r, b_g) \gets $ Interact with caregiver with mode $\chi_i$. }
\ELSIF{$\chi_i$ is an Auton. Exploration learning mode}
  \STATE{ $(a_r,b_r, b_g) \gets $ Perform action with mode $\chi_i$. }
\ENDIF
    \STATE{ \textbf{Learning: }  Update $p$} with $(a_r,b_r)$.
        \STATE{$\gamma \gets$ Competence for $b_g$  }
\UNTIL{end of trials for the same object}	  


%  \STATE{ $\mathcal{R } \gets $ Update $\textsf{Goal Interest Mapping}(\mathcal{R },\mathcal{H},b_g,\gamma)$}
  \STATE{\textbf{Meta-Learning: }  $\mathcal{R } \gets $ Update $\textbf{Goal Interest Mapping}(\mathcal{R },\mathcal{H},b_g,\gamma)$}
\ENDLOOP	  
\end{algorithmic}
\end{algorithm}


==> pseudocode/PseudoCodeSGIMD.tex <==
\begin{algorithm}
\caption{SGIM-D}
\zlabel{alg:PseudoCodeSGIMD}
\begin{algorithmic}[1]
\STATE  {\bfseries Initialization:} $\mathcal{R } \gets $  singleton ${C \times A}$
\STATE  {\bfseries Initialization:} Initalise $p_1$ to a homogeneous probability density
\STATE  {\bfseries Initialization:} $\mathcal{H} \gets$  empty episodic memory (collection of episodes of reached outcome $a$ with policy parameter $b$ in context $c$, $(c,b,a)$) 
%\STATE  {\bfseries Initialization:} $ e \gets 1$

\LOOP
\STATE{ Retrieve sampling mode $\chi$}
  \IF{$\chi = Imitation $}
  \STATE{\textbf{\underline{Social Learning Mode}}}
\REPEAT
  \STATE{$(a_{d}, b_{d}, c_{d}) \gets \textsf{ Correspondence} $ of the teacher's demonstration } \zlabel{line:correspondance}
  \STATE{\textsf{Emulate Goal}: $a_g \gets a_{d}$  \zlabel{line:emulate}}
          \STATE{ $\mathcal{D} \gets$ {\textsf{Mimic Policy}} ($b_{d},c$) }
    \STATE $p \gets \mathcal{L}(p,\mathcal{D})$  
\UNTIL{End of social interaction}

  \ELSE
  \STATE{ \textbf{\underline{Intrinsic Motivation Mode}}}
       \STATE{Measure current context $c$}	
       \STATE{$a_g \gets $ \textsf{Decide a goal} with a probability proportional to its associated expected competence progress   \zlabel{line:decideGoal}}
       
	\REPEAT

	         \STATE{ $\mathcal{D} \gets {\textsf{Goal-Directed Policy Optimisation}}(c,a_g, p, \mathcal{H})$  }
    \STATE $p \gets \mathcal{L}(p,\mathcal{D}) $ 

	      	       
\UNTIL{Terminate reaching of $a_g$}
\ENDIF

\STATE{ Append $\mathcal{D} $ to $\mathcal{H}$ }
  \STATE{ $\mathcal{R } \gets $ Update $\textsf{Goal Interest Mapping}(\mathcal{R },\mathcal{H},c,a_g)$   \zlabel{line:goalInterestMappingSGIMD}}
\ENDLOOP	  
\end{algorithmic}
\end{algorithm}

==> pseudocode/PseudoCodeSGIMIM.tex <==
\begin{algorithm}
\caption{SGIM-IM}
\zlabel{alg:PseudoCodeSGIMIM}
\begin{algorithmic}[1]
%\STATE {{\bfseries Input:} $nbImitate$ : duration of the imitation phase;}
%\STATE {{\bfseries Input:} thresholds:  $\epsilon_{max}$; }
%\STATE {\bfseries Initialization:} rest position $(x_{org}, y_{org})$.
%\STATE {\bfseries Input:} $p_1, p_2, p_3$ as probabilities of methods for choosing a goal in the task space by the Goal Self-Generation Module (totally random, random goal in the most interesting region, worst mastered goal in the most interesting region)  
\STATE  {\bfseries Initialization:} $\mathcal{R } \gets $  singleton $C \times A$
%\STATE  {\bfseries Initialization:} $flagInteraction  \gets false$
\STATE  {\bfseries Initialization:} $\mathcal{H} \gets$  empty episodic memory (collection of episodes (c,b,a))
\STATE  {\bfseries Initialization:} $\Delta_S$ : progress values made by social guidance mode
\STATE  {\bfseries Initialization:}  $\Delta_A$ : progress values made by intrinsic motivation  mode
\STATE  {\bfseries Initialization:} $e \gets 1$

\LOOP
\STATE{ $\chi_e \gets \textsf{Select Sampling Mode}(\Delta_S,\Delta_A)$}  \zlabel{line:stochasticBehaviour}
  \IF{$\chi_e == \chi_{demo} $}
  \STATE{\textbf{\underline{Social Learning Mode}}}
  \STATE{ demo $\gets$ ask and perceive demonstration }
  \STATE{$(c_{d}, b_{d}, a_{d}) \gets \textsf{ Correspondence} $ (demo)}
  \STATE{\textsf{Emulate Goal}: $a_g \gets a_{d}$ }%and the context $c \gets c_{demo}$ }
             \STATE{$\gamma_i \gets$ Competence for $a_g$  } \zlabel{line:competencei_soc}

        \STATE{$ \mathcal{D}_e  \gets {\textsf{Mimic Policu}} (b_{d}$) }
            \STATE{$\gamma \gets$ Competence for $a_g$  }  \zlabel{line:competencef_soc}
                \STATE $p_{e+1} \gets \mathcal{L}(p_e,\mathcal{D}_e)$ 
         \STATE{Add $\gamma - \gamma_i$ to stack $\Delta_S$}   \zlabel{line:progress_soc}

  \ELSE
  \STATE{ \textbf{\underline{Intrinsic Motivation Mode}}}
       \STATE{$a_g \gets \textsf{Decide a goal}( \mathcal{R })$}
           \STATE{$\gamma_i \gets$ Competence for $a_g$  }   \zlabel{line:competencei_aut}

	\REPEAT

	         \STATE{ $\mathcal{D}_e   \gets {\textsf{Goal-Directed Policy Optimisation}}(a_g) $}
    \STATE $p_{e+1} \gets \mathcal{L}(p_e,\mathcal{D}_e)$ 

	      	       
\UNTIL{Terminate reaching of $a_g$}
    \STATE{$\gamma \gets$ Competence for $a_g$  }  \zlabel{line:competencef_aut}

         \STATE{ Add $\gamma - \gamma_i$ to stack $\Delta_A$ }   \zlabel{line:progress_aut}
\ENDIF

\STATE{ Append $\mathcal{D}_e $ to $\mathcal{H}$ }
  \STATE{ $\mathcal{R } \gets $ Update $\textsf{Goal Interest Mapping}(\mathcal{R },\mathcal{H},c,a_g)$   \zlabel{line:goalInterestMappingSGIMIM}}
\STATE{$e \gets e+1$}

\ENDLOOP	  
\end{algorithmic}
\end{algorithm}

==> pseudocode/PseudoCodeSelectLabelStrategyIcub.tex <==
\begin{algorithm}
\caption{ [$\chi,b_g$] = Select Label And Sampling Mode($\mathcal{R }$ ) }
 \zlabel{alg:SelectLabelStratIcub}
\begin{algorithmic}[1]
\STATE {\bfseries input:} $\mathcal{R}$: set of regions $R_n$ and corresponding $interest_{R_n}(\chi)$ for each strategy $\chi$.
\STATE{\bfseries parameters:} $ 0 \leq p_1 \leq 1$ : probability for random mode.
\STATE{$p \gets$ random value between 0 and 1.}
\IF{$p<p_1$ }
\STATE{ Ensure a minimum of exploration, i.e. :  }  \zlabel{line:selectStochRandomIcub}
\STATE {Choose $\chi$ and $b_g \in B$ randomly }
\ELSE 
\STATE{Focus on areas of highest competence progress, i.e. :}  \zlabel{line:selectStochInterestIcub}
\STATE{$\forall (\chi,n$), $P_n(\chi) \gets \frac{ interest_{R_n}(\chi) - \textbf{min}(interest_{R_i})}{\sum_{i=1}^{|R_n|}interest_{R_i}(\chi) - \textbf{min}(interest_{R_i})}$}

\STATE{$(b,\chi) \gets argmax_{n,\chi} P_n(\chi) $}
\ENDIF

\RETURN  $(b,\chi)$
\end{algorithmic}
\end{algorithm}


==> pseudocode/PseudoCodeSelectRegimeIM.tex <==
\begin{algorithm}
\caption{[$\chi$] = SelectSamplingMode($\Delta_S,\Delta_A$)}
\zlabel{alg:PseudoCodeRegimeSelection}
\begin{algorithmic}
\STATE { {\bfseries input}:  $\Delta_S$ : progress values made by social learning Mode}
\STATE { {\bfseries input}:  $\Delta_A$ : progress values made by intrinsic motivation learning Mode}
\STATE { {\bfseries output}: $\chi$ : chosen Mode}
\STATE { {\bfseries parameter}: $nbMin$ : duration of the initiation phase}
\STATE { {\bfseries parameter}: $ns$ : window frame for monitoring progress}
\STATE { {\bfseries parameter}: $cost$ : cost of requesting a demonstration}

\STATE{\textbf{\underline{Initiation phase}}}
\IF{ Social Learning and Intrinsic Motivation Modes have not been chosen each $nbMin$ times yet}
\STATE{$ps \gets 0.5$}
\ELSE
\STATE{\textbf{\underline{Permanent phase}}}
\STATE{$wa \gets$ average(last $ns$ elements of $\Delta_A$)}  \zlabel{line:prefAverageAut}
\STATE{$ws \gets \frac{average(\textsf{last }ns \textsf{elements of } \Delta_S)}{cost}$} \zlabel{line:prefAverageDem}
\STATE{ $ps \gets min(0.9, max(0.1, \frac{ws}{ws + wa} ))$}
\ENDIF

\STATE{$\chi \gets \chi_{dem}$  with probability $ps$}  \zlabel{line:stochasticMode}
\RETURN{$\chi$}

\end{algorithmic}
\end{algorithm}

==> pseudocode/PseudoCodeUpdateRegionsACTS.tex <==
\begin{algorithm}
\caption{ [$\mathcal{R}$] =  Update Outcome and Sampling Mode Interest Mapping($\mathcal{R },\mathcal{H},a_g,progress_g, \chi$) }
\zlabel{alg:UpdateRegions}
\begin{algorithmic}
\STATE {\bfseries input:} $\mathcal{R}$: set of regions $R_n$ and corresponding $interest_{R_n}(\chi)$ for each sampling mode $\chi$.
\STATE {\bfseries input:} $a_g, progress_g$: goal outcome of the episode and its progress measure.
\STATE {\bfseries input:} $\mathcal{H}$: the set of all observed outcomes during the episode and their progress measures $(a_r, progress_r)$.
\STATE {\bfseries input:} $\chi$: sampling mode and teacher used during the episode.

\STATE {\bfseries parameter:} $g_{Max}$ : the maximal number of elements inside a region.
\STATE {\bfseries parameter:} $\delta$ : a time window used to compute the interest.
\FOR{all $ (a,progress) \in \{\mathcal{H}, (a_g, progress_g)\}$ }
\STATE{Find the region $R_n \in \mathcal{R}$ such that $a \in R_n$.}
\STATE{Add $progress$ in $R_n(\chi)$, the list of competence progress measures of experiments $ a \in R_n$ with sampling mode $\chi$.}
\STATE{Compute the new value of  competence progress of $R_n(\chi)$: } 
\begin{center}
\STATE{$interest_{R_n}(\chi) = \frac{\displaystyle mean_{i=|{R}_n|-\delta}^{|{R}_n|} progress_{i}}{ \kappa (\chi) } $}
\end{center}
\IF{ $|R_n(\chi)| > g_{max}$}   \zlabel{line:ACTSTriggerSplit}
\STATE{ $\mathcal{R} \gets$ Split $R_n$. } \zlabel{line:ACTSSplit}
\ENDIF
\ENDFOR
\RETURN $\mathcal{R}$
\end{algorithmic}
\end{algorithm}


==> pseudocode/PseudoCodeUpdateRegionsIcub.tex <==
%\begin{algorithmbis}[\textbf{ [$\mathcal{R}$] = GoalInterestMapping}($\mathcal{R },\mathcal{H},b,\gamma$) ] \zlabel{alg:UpdateRegions}
\begin{algorithm}
\caption{ [$\mathcal{R}$] = Goal Interest Mapping($\mathcal{R },\mathcal{H},b,\gamma$) }
\zlabel{alg:UpdateRegionsIcub}
\begin{algorithmic}[1]
\STATE {\bfseries input:} $b$: set of objects and corresponding $interest(b,\chi)$ for each strategy $\chi$.
\STATE {\bfseries input:} $\delta$ : a time window used to compute the interest.
\STATE{Add $\gamma$ to $R(b,\chi)$, the list of competence measures for object $b \in B$ with strategy $\chi$.}
\STATE{Compute the new value of  competence progress of $b$: } 
\begin{center}
\STATE{$interest(b,\chi)  = \frac{1}{\kappa (\chi)} \frac{ \left| \left(\displaystyle \sum_{j=N-\delta}^{N-\frac{\delta}{2}} \gamma_{j} \right) - \left(\displaystyle \sum_{j=N-\frac{\delta}{2}}^{N} \gamma_{j} \right) \right|}{\delta} $}
\end{center}
%\IF{ $|R_n(\chi)| > g_{max}$}
%\STATE{ $\mathcal{R} \gets$ Split $R_n$ into 2 so as to maximise the difference in interest measures between the 2 subspaces. }
%\ENDIF
\RETURN $\mathcal{R}$ the set of all $R(b,\chi)$
\end{algorithmic}
\end{algorithm}


==> pseudocode/PseudoCodeUpdateRegionsSGIMD.tex <==
\begin{algorithm}
\caption{ [$\mathcal{R}$] = UpdateRegions($\mathcal{R}, (c,a),\gamma$) ]}
\zlabel{alg:UpdateRegionsSGIMD}
\begin{algorithmic}[1]
\STATE {\bfseries input:} $\mathcal{R}$: set of regions and corresponding $interest$.
\STATE {\bfseries input:} $(c,a)$: context and effect of the learning exemplar.
\STATE {\bfseries input:} $\gamma$: competence at reaching $a$ in context $c$.
\STATE {\bfseries parameter}: $g_{Max}$ : the maximal number of elements inside a region.
\STATE {\bfseries parameter:} $\zeta$ : a time window used to compute the interest.
\STATE{Find the region $R_n \in \mathcal{R}$ such that $(c,a) \in R_n$.}
\STATE{Add $\gamma$ to $R_n$.}
\STATE{Compute the new value of $interest_n$ of $R_n$ according to each $(c_i,a_i) \in R_n$ of competence $\gamma_i$ such that:} 
\begin{center}
\STATE{$interest_n =  \frac{\left| \left(\displaystyle \sum_{i=| {R}_n|-\zeta}^{|{R}_n|-\frac{\zeta}{2}} \gamma_{i} \right) - \left(\displaystyle \sum_{i=|{R}_n|-\frac{\zeta}{2}}^{|{R}_n|} \gamma_{i} \right) \right|}{\zeta}$}
\end{center}
\IF{ $|R_n| > g_{max}$}
\STATE{Split $R_n$. }
\ENDIF
\RETURN $\mathcal{R}$
\end{algorithmic}
\end{algorithm}

